Mutations of group species with potentials and their representations. Applications to cluster algebras

This article tries to generalize former works of Derksen, Weyman and Zelevinsky about skew-symmetric cluster algebras to the skew-symmetrizable case. We introduce the notion of group species with potentials and their decorated representations. In good cases, we can define mutations of these objects in such a way that these mutations mimic the mutations of seeds defined by Fomin and Zelevinsky for a skew-symmetrizable exchange matrix defined from the group species. These good cases are called non-degenerate. Thus, when an exchange matrix can be associated to a non-degenerate group species with potential, we give an interpretation of the $F$-polynomials and the $\g$-vectors of Fomin and Zelevinsky in terms of the mutation of group species with potentials and their decorated representations. Hence, we can deduce a proof of a serie of combinatorial conjectures of Fomin and Zelevinsky in these cases. Moreover, we give, for certain skew-symmetrizable matrices a proof of the existance of a non-degenerate group species with potential realizing this matrix. On the other hand, we prove that certain skew-symmetrizable matrices can not be realized in this way.

==> exemple.tex <==
The aim of this part is to show an example where the technique shown in the previous sections works and a counterexample where there is no non-degenerate potential.

\makeatletter
\newcommand*{\contains}[2]{%
  \TE@throw
  \noexpand \in@ {#2}{#1}%
  \noexpand \ifin@
}

\newcommand*{\tempb}{}

\newcommand*{\tri}[1]{%
    \renewcommand*{\tempb}{}%
    \@for \tempa :=#1\do {%
    \ifthenelse{\contains{#1}{GD}}%
      {\protected@edef \tempb {\tempb ,"A1";"A2"**\string @{-},?>*\string @{>}}}{}% 
    \ifthenelse{\contains{#1}{DG}}%
      {\protected@edef \tempb {\tempb ,"A2";"A1"**\string @{-},?>*\string @{>}}}{}% 
    \ifthenelse{\contains{#1}{GB}}%
      {\protected@edef \tempb {\tempb ,"A1";"A3"**\string @{-},?>*\string @{>>}}}{}% 
    \ifthenelse{\contains{#1}{BG}}%
      {\protected@edef \tempb {\tempb ,"A3";"A1"**\string @{-},?>*\string @{>>}}}{}%
    \ifthenelse{\contains{#1}{DB}}%
      {\protected@edef \tempb {\tempb ,"A2";"A3"**\string @{-},?>*\string @{>>}}}{}% 
    \ifthenelse{\contains{#1}{BD}}%
      {\protected@edef \tempb {\tempb ,"A3";"A2"**\string @{-},?>*\string @{>>}}}{}%  
    }%
    \protected@edef \tempb ##1##2{##1\tempb##2}%
    \tempb {\begin{xy} 0;<1pc,0pc>:, {\xypolygon3"A"{~*{\ifcase\xypolynode\or \cdot \or \cdot \or \bullet \fi }~>{} }}}{\end{xy}}}

\newcommand*{\trig}[4]{%
    \renewcommand*{\tempb}{}%
    \@for \tempa :=#4\do {%
    \ifthenelse{\contains{#4}{GD}}%
      {\protected@edef \tempb {\tempb ,"A1";"A2"**\string @{-},?>*\string @{>}}}{}% 
    \ifthenelse{\contains{#4}{DG}}%
      {\protected@edef \tempb {\tempb ,"A2";"A1"**\string @{-},?>*\string @{>}}}{}% 
    \ifthenelse{\contains{#4}{GB}}%
      {\protected@edef \tempb {\tempb ,"A1";"A3"**\string @{-},?>*\string @{>>}}}{}% 
    \ifthenelse{\contains{#4}{BG}}%
      {\protected@edef \tempb {\tempb ,"A3";"A1"**\string @{-},?>*\string @{>>}}}{}%
    \ifthenelse{\contains{#4}{DB}}%
      {\protected@edef \tempb {\tempb ,"A2";"A3"**\string @{-},?>*\string @{>>}}}{}% 
    \ifthenelse{\contains{#4}{BD}}%
      {\protected@edef \tempb {\tempb ,"A3";"A2"**\string @{-},?>*\string @{>>}}}{}%  
    }%
    \protected@edef \tempb ##1##2{##1\tempb##2}%
    \tempb {\begin{xy} 0;<1.5pc,0pc>:, {\xypolygon3"A"{~*{\ifcase\xypolynode\or #1 \or #2 \or #3 \fi }~>{} }}}{\end{xy}}}

\makeatletter

\begin{figure}
 {
 $$\begin{xy}
    		0;<0pc,3.468pc>:,="D",
   		{\xypolygon4"A"{~*{\ifcase\xypolynode\or \tri{GD DB} \or \tri{GD BD} \or \tri{DG BD} \or \tri{DG DB} \fi }~:{(1,0):}~>{}}},
   		{\xypolygon4"B"{~*{\ifcase\xypolynode\or \tri{DG GB BD} \or \tri{DG DB} \or \tri{GD DB BG} \or \tri{GD BD} \fi}~:{(2.12132,0):}~>{}}}, %3/sqrt2
    		{\xypolygon6"C"{~*{\ifcase\xypolynode\or \tri{BG GD} \or \tri{GD DB BG} \or \tri{DG BD} \or \tri{DG GB} \or \tri{DG GB BD} \or \tri{GD DB} \fi}~:{(3,0):}~>{}}},
		{\xypolygon12"D"{~*{\ifcase\xypolynode\or \tri{GD GB} \or \tri{DG BG} \or \tri{DG GB} \or  \or  \or \or \tri{DG BG} \or \tri{GD GB} \or \tri{BG GD} \or \or \or \fi}~:{(4.098,-1.098):}~>{}}},
    		"A1";"A2"**\dir{-},
		"A2";"A3"**\dir{-},
    		"A3";"A4"**\dir{-},
		"A4";"A1"**\dir{-},
		"A1";"B1"**\dir{-},
		"A2";"B2"**\dir{-},
		"A3";"B3"**\dir{-},
		"A4";"B4"**\dir{-},
		"B1";"C1"**\dir{-},
		"B1";"C2"**\dir{-},
		"B2";"C3"**\dir{-},
		"B2";"C4"**\dir{~},
		"B3";"C4"**\dir{-},
		"B3";"C5"**\dir{-},
		"B4";"C6"**\dir{-},
		"B4";"C1"**\dir{~},
		"C2";"C3"**\dir{-},
		"C5";"C6"**\dir{-},
		"D1";"C1"**\dir{-},
		"D1";"C6"**\dir{~},
		"D7";"C4"**\dir{-},
		"D7";"C3"**\dir{~},
		"D1";"D2"**\dir{-},
		"D2";"D3"**\dir{-},
		"C2";"D3"**\dir{-},
		"D7";"D8"**\dir{-},
		"D8";"D9"**\dir{-},
		"C5";"D9"**\dir{-},
		"D3";"D8"**\crv{(-3,5)&(-5,0)},
		"D9";"D2"**\crv{(5,-5)&(7,0)},
    \end{xy}$$
 }
 \caption{Exchange graph of type $B_3$} \label{figeg}
\end{figure}
\makeatother

Suppose here that $K = \C$. We fix $\Gamma_1 = \Gamma_2$ to be the trivial group and $\Gamma_3 = \Z/2\Z$. We take $A_{12} = \C$ and $A_{23} = \C[\Z / 2\Z]$, the other $A_{ij}$ vanishing. Then $A$ is acyclic and therefore $S = 0$ is a non-degenerate potential, in view of section \ref{nondeg}. Moreover,
 $$B(A) = \left( \begin{matrix}
  0 & -1& 0 \\
  1 & 0 & -1 \\
  0 & 2 & 0
 \end{matrix}\right)$$
 which is of type $C_3$. Its exchange graph is given on figure \ref{figeg} where the small dots ($\cdot$) symbolize vertices with trivial group and big dots ($\bullet$) symbolize vertices with group $\Z/2\Z$. Simple arrows symbolize $\C$ and double arrows symbolize $\C[\Z/2\Z]$. Thus, $(A, S)$ will be symbolized by 
$$\tri{GD DB}.$$
 Finally, wave lines ($\sim$) symbolize mutations composed with the exchange of vertices $1$ and $2$.

 Now, we will compute explicitly $F^B_{3;213}$ and $\g^B_{3;213}$. We will follow the construction of section \ref{fpol}. According to the exchange graph,
 $$\mu_3 \mu_1 \mu_2(A, 0) = \left(\tri{GD GB}, 0\right) = (A', S').$$
 Let $\rho$ be one the two irreducible modules over $\Z/2\Z$. Then
 $$\mu_3(A', S', 0, \rho) = \left(\tri{GD BG}, 0, \trig{0}{0}{\rho}{}, 0 \right)$$
 $$\mu_1 \mu_3(A', S', 0, \rho) = \left(\tri{DG GB BD}, \dots, \trig{\C}{0}{\rho}{GB}, 0 \right)$$
 $$\mu_2 \mu_1 \mu_3(A', S', 0, \rho) = \left(\tri{GD DB}, \dots, \trig{\C}{\C}{\rho}{GD DB}, 0 \right)$$
 (the arrows are obvious) and therefore,
 $$X^B_{\rho;213} = \trig{\C}{\C}{\rho}{GD DB}$$
 which induces that:
 $$F_{X^B_{\rho;213}} = 1 + Y_\rho + Y_2 Y_\rho + Y_1 Y_2 Y_\rho$$
 and therefore
 $$\check F_{X^B_{\rho;213}} = 1 + Y_3 + Y_2 Y_3 + Y_1 Y_2 Y_3.$$
 Moreover,
 $$\g_{X^B_{\rho;213}} = \left( \begin{matrix} 0 \\ 0 \\ -\rho \end{matrix} \right)$$
 and therefore 
 $$\check \g_{X^B_{\rho;213}} = \left( \begin{matrix} 0 \\ 0 \\ -1 \end{matrix}\right).$$
 It is easy to check by hand that these coincide with $F^B_{3;213}$ and $\g^B_{3;213}$ obtained for example by formulas of \cite[\S 2]{DeWeZe}.

Let now $B$ be the matrix defined by
$$B = \left( \begin{matrix}
 0 & 0 & 1 & 1 & -1 & -2 \\
 0 & 0 & -1 & -1 & 1 & 2 \\
 -1 & 1 & 0 & 0 & 0 & 0 \\
 -1 & 1 & 0 & 0 & 0 & 0 \\
 1 & -1 & 0 & 0 & 0 & 0 \\
 1 & -1 & 0 & 0 & 0 & 0 
\end{matrix} \right).
$$

We will show that there is no non-degenerate locally free GSP with mutation matrix $B$. Suppose that $(I, (\Gamma_i), A, S)$ is a non-degenerate GSP with mutation matrix $B$. Then, $\Gamma_1$, \dots, $\Gamma_5$ have the same cardinal which is two times the one of $\Gamma_6$. Applying $\mu_3$ followed by $\mu_5$ create $2$-cycles and implies, in view of proposition \ref{eff2c}, that 
 $$A_{23} \tens_{E_3} A_{31} \simeq \left(A_{15} \tens_{E_5} A_{52}\right)^*.$$
In the same way, applying $\mu_4$ followed by $\mu_5$ implies that
 $$A_{24} \tens_{E_4} A_{41} \simeq \left(A_{15} \tens_{E_5} A_{52}\right)^*.$$
With the same type of argument, applying $\mu_3$, $\mu_4$ and $\mu_6$ implies that
 $$\left(A_{23} \tens_{E_3} A_{31}\right)^{\oplus 2} \simeq A_{24} \tens_{E_4} A_{41} \oplus A_{23} \tens_{E_3} A_{31} \simeq \left(A_{16} \tens_{E_6} A_{62}\right)^*.$$
As all considered groups are semisimple, it is easy to see that the $(E_1, E_6)$-bimodule $A_{16}$ can be decomposed as a direct sum of
the form
 $$A_{16} = \bigoplus_{i = 1}^m r_i \tens_K s_i$$
where the $r_i$ are irreducible left $E_1$-modules and the $s_i$ are irreducible right $E_6$-modules. Moreover, the $r_i \tens_K s_i$ are irreducible bimodule and satisfy, because of $B$, 
 $$\forall r \in \irr_1, \sum_{i\,|\, r_i \simeq r} \dim_K s_i = \dim_K r \text{ and } \forall s \in \irr_6, \sum_{i\,|\, s_i \simeq s} \dim_K r_i = 2 \dim_K s.$$
 Thus, there are exactly two indices which can be supposed to be $1$ and $2$ such that $s_1$, $s_2$ are trivial and $r_1$ and $r_2$ are of dimension $1$ and appear only one time in the sequence $(r_i)$.
 In the same way,
 $$A_{62} = \bigoplus_{i = 1}^n t_i \tens_K u_i$$
 with
 $$\forall t \in \irr_6, \sum_{i\,|\, t_i \simeq t} \dim_K u_i = 2 \dim_K t  \text{ and } \forall u \in \irr_2, \sum_{i\,|\, u_i \simeq u} \dim_K t_i = \dim_K u.$$
 Thus, there are exactly two indices which can be supposed to be $1$ and $2$ such that $t_1$, $t_2$ are trivial and the $u_1$ and $u_2$ are of dimension $1$ and appear only one time in the sequence $(u_j)$.
 Hence, 
 $$\left(A_{16} \tens A_{62}\right)^* = \mathop{\bigoplus_{i = 1}^m \bigoplus_{j = 1}^n}_{s_i \simeq t_j^*} \left(u_j^* \tens_K r_i^*\right)^{\dim_K s_i}$$
 contains $u_1^* \tens r_1^* \oplus u_1^* \tens r_2^* \oplus u_2^* \tens r_1^* \oplus u_2^* \tens r_2^*$ as the only summands containing $u_1^*$, $u_2^*$, $r_1^*$ and $r_2^*$. Finally, $\left(A_{16} \tens A_{62}\right)^*$ can not be decomposed as a direct sum of two times the same bimodule, which is a contradiction.

